Equilibrium Finding in Normal-Form Games Via Greedy Regret Minimization

We extend the classic regret minimization framework for approximating equilibria in normal-form games by greedily weighing iterates based on regrets observed at runtime. Theoretically, our method retains all previous convergence rate guarantees. Empirically, experiments on large randomly generated games and normal-form subgames of the AI benchmark Diplomacy show that greedy weights outperforms previous methods whenever sampling is used, sometimes by several orders of magnitude.

==> paper/abandoned.tex <==

\section{Old Bad Proof}
Denote our player as $i$. \pyear{brown2019solving}, which in turn references \pyear{cesa2006prediction}, bounds the regret of weighted regret minimization, where iteration $t$ is given weight $w_t$, as \[
R_i^{w, T} \leq \frac{\triangle \sqrt{\lvert A \rvert} \sqrt{\sum_{t=1}^T w_t^2}}{\sum_{t=1}^T w_t}
\]
Because every weight chosen by Algorithm~\ref{mainalgorithm} will satisfy $1 \leq w_t \leq M$ by construction, we can immediately bound the right hand side with 
\[
\frac{\triangle \sqrt{\lvert A \rvert} \sqrt{\sum_{t=1}^T w_t^2}}{\sum_{t=1}^T w_t} \leq \frac{\triangle M \sqrt{\lvert A \rvert}}{\sqrt{T}} = O\left(\frac{1}{\sqrt{T}}\right)
\]

==> paper/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our work is a general method for solving games. While general methods can always be used for both beneficial and harmful purposes, we believe our work to too broadly applicable to discuss specific negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:approach}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:approach} and Appendix~\ref{sec:mainpropproof}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code will be uploaded in supplementary materials.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We give a detailed report in the experimental section and include the code for most experiments in the supplementary materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report $95\%$ confidence intervals on all the major experimental results.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:experiments}. Our experiments did not require substantial computational resources. Random matrix experiments were run on a single CPU core of a Macintosh laptop. Diplomacy experiments were run on a single CPU core and a single NVIDIA V100 GPU. We described the resources in Section~\ref{sec:experiments}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> paper/related.tex <==
\section{Related Work}
\subsection{Weighting Schemes}
While the original regret minimization framework proposed by \pyear{blackwell1956analog} and \pyear{hannan1957approximation} weight all iterations of the regret minimization procedure equally, some recent work has explored the idea of weighting different iterations differently. \pyear{brown2019solving} gives convergence rate bounds and runs experiments for several (fixed) weighting schemes for the regret minimization and show that empirically, this can also lead to speed improvements in many large, sequential, two-player zero-sum games. Our work generalizes this concept by allowing the procedure itself to determine the weighting of each iteration \emph{at runtime} and extending the experiments to games with more than two players and with general sum payoff functions.
\subsection{Improving Regret Minimization}
A substantial amount of work over the last decade has focused on improving (external) regret minimization techniques in two-player zero-sum games, with a special eye towards the variant of regret minimization for large sequential games: CFR \citep{zinkevich2008regret}. We examine several of these variants, including CFR+ \citep{tammelin2014solving}, Linear CFR \citep{brown2019solving}, optimism \citep{syrgkanis2015fast}, and alternating updates \citep{tammelin2014solving} and describe their inner workings in more detail in Sections~\ref{sec:approach} and \ref{sec:experiments}.
\subsection{Correlated Equilibria}
The correlated equilibrium is one of the leading solution concepts for multiplayer games. Unlike the Nash equilibrium, it requires some sort of correlated device or common source of randomness seen by all players. However, in exchange and unlike the Nash equilibrium solution concept, it is computationally tractable and furthermore can be learned via simple procedures that are plausible for real-world agents to follow \citep{hart2000simple}. Recent work has extended such results to large sequential games, where players can undertake multiple moves in sequence instead of all moving simultaneously \citep{celli2020no}. We leave to future work whether greedy weights can be applied to accelerate regret minimization in such sequential games.
While polynomial time algorithms based on linear programming have long been known for computing correlated equilibria \citep{papadimitriou2008computing}, they are relatively slow in practice. This is because, in practice, regret minimization is sublinear with respect to the matrix, while other methods are polynomial at best.
\subsection{Sampled Strategies v. Monte Carlo CFR}
Our requirement that players play pure strategies at each iteration is related but not identical, to prior work using Monte-Carlo methods for regret minimization (e.g. MC-CFR) \citep{lanctot2009monte, lanctot2013monte}. In MC-CFR, players play a mixed strategy at each timestep, but their regrets are estimated via sampling outcomes rather than computed exactly. As such, the calculated regrets serve only as an approximation of the true regrets. When requiring each iteration to consist of pure strategies, the sampling takes place on the player's side in that they must sample a pure strategy to play, after which they receive their exact regrets based on what they actually played. As such, the regrets we calculate are exact and if the maximum internal regret of any player is $\epsilon$, then we immediately have a $2\epsilon$-correlated equilibria.
\subsection{Relationship to Online Machine Learning}
Regret minimization has many applications to (and has drawn many lessons from) other fields including online machine learning and predictions of arbitrary sequences. In particular, past work has demonstrated very strong relationships between the concepts of regret minimization and online machine learning \citep{cesa2006prediction, abernethy2011blackwell}.

In our application of discovering equilibria in games, we allow the procedure itself to determine the weight of each iterations. Note that in other settings where regret minimization might be applied (e.g. sequence prediction), this would \emph{not} be a reasonable allowance because it would be akin to upweighting low regret iterations (where you predicted correctly) and downweighting times when you made a mistake. However, in the self play setting for discovering the equilibria of games, each ``agent'' is a construction we use to find equilibria and we are thus uninterested in any given agent's performance, only that the overall regret of the algorithm goes to 0 as quickly as possible. As a result, we do precisely what we would not be allowed to do in any online machine learning setting: we upweight iterations that minimize overall regret for agents in the game, and downweight those that do not.
